A Datalog-based Computational Model for Coordination-free, Data-Parallel Systems

Cloud computing refers to maximizing efficiency by sharing computational and storage resources, while data-parallel systems exploit the resources available in the cloud to perform parallel transformations over large amounts of data. In the same line, considerable emphasis has been recently given to two apparently disjoint research topics: data-parallel, and eventually consistent, distributed systems. Declarative networking has been recently proposed to ease the task of programming in the cloud, by allowing the programmer to express only the desired result and leave the implementation details to the responsibility of the run-time system. In this context, we propose a study on a logic-programming-based computational model for eventually consistent, data-parallel systems, the keystone of which is provided by the recent finding that the class of programs that can be computed in an eventually consistent, coordination-free way is that of monotonic programs. This principle is called CALM and has been proven by Ameloot et al. for distributed, asynchronous settings. We advocate that CALM should be employed as a basic theoretical tool also for data-parallel systems, wherein computation usually proceeds synchronously in rounds and where communication is assumed to be reliable. It is general opinion that coordination-freedom can be seen as a major discriminant factor. In this work we make the case that the current form of CALM does not hold in general for data-parallel systems, and show how, using novel techniques, the satisfiability of the CALM principle can still be obtained although just for the subclass of programs called connected monotonic queries. We complete the study with considerations on the relationships between our model and the one employed by Ameloot et al., showing that our techniques subsume the latter when the synchronization constraints imposed on the system are loosened.

==> datalog.tex <==
In this work, we will always use \emph{Datalog$^{\neg}$} to express queries.
%Let \textbf{var} be infinite set of \textit{variables} used to range over the elements of \textbf{dom}, and disjoined both from \textbf{dom} and \textbf{relname}
%Given a relation name $R$ and related arity $k$, a \emph{free tuple} over $R$ is an ordered $k$-tuple composed by only constants and variables.
%An \textit{atom} over $R$ is an expression in the form $R(u_1, \ldots, u_k)$ where each $u_i$ is referred to as a \emph{term}. 
%In the following we will use interchangeably the terms \textit{relations} and \textit{predicates}. 
%A \textit{literal} is an atom -- in this case we refer to it as \textit{positive} -- or the negation of an atom. 
%Now, a \textit{ground atom} %or equivalently a \textit{fact},
%is an atom containing only constant terms -- i.e., $u_i \in$ \textbf{dom}.
%
A Datalog$^\neg$ rule is an expression in the form:
\vspace{-1mm}
\begin{equation}
H(\bar{w}) \leftarrow B_1(\bar{u}_1), \ldots, B_n(\bar{u}_n), \neg C_1(\bar{v}_1), \ldots, \neg C_m(\bar{v}_m).
\end{equation}
%
where $H$, $B_i$, $C_j$ are relation names and $\bar{w}, \bar{u}_i, \bar{v}_j$ are tuples of appropriate arity. As usual $H(\bar{w})$ is referred to as the \textit{head}, and $B_1(\bar{u}_1)$, \ldots, $C_m(\bar{v}_m)$ as the \textit{body}. 
%If $m = 0$ the rule is \textit{positive} and expresses a \textit{definite clause}, while if $m=n=0$ the rule is expressing a \textit{fact} (\textit{clause}). 
%Note that predicates appearing in the body of a rule can also be used in the head of the same rule to produce \emph{recursive} computation. 
We allow \textit{built-in} predicates to appear in the bodies of rules, i.e., we allow relation names such as $=$,$\ne$,$\leqslant$, $<$, $\geqslant$, and $>$, each of them having their natural meaning.
%
%as well as relations for arithmetic operations such as $+$ and operations of string values. 
%
%To be consistent with the standard notation, we use the infix notation and write $X \ge Y$ instead of $\ge$$(X, Y )$. 
%
%Similarly, we write $X + Y = Z$ instead of $+(X, Y, Z)$. 
%All these symbols are always interpreted in the standard way. 
We also allow \textit{aggregate relations} in positive rule-heads in the form $R(\bar{u}, \Lambda <w>)$, with $\Lambda$ one of the usual aggregate functions, $w$ a variable from the body, and $\bar{u}$ is a list thereof, called the grouping variables. %\cite{DBLP:journals/jlp/RamakrishnanU95}.
We allow two different types of aggregate functions: \emph{stratified aggregates}, with the usual semantics, and \emph{monotonic aggregates} as defined in \cite{DBLP:journals/vldb/MazuranSZ13}.
In order to differentiate between monotonic and stratified aggregation functions, we label the former with the $fs$ (\emph{frequency support}) prefix as specified in Zaniolo's work.

%Mumick and Shmueli ob- serve correspondences in the expressivity of Datalog with stratified negation and strati- fied aggregation functions [Mumick,I.S.,Shmueli,O.:Howexpressiveisstratifiedaggregation?]. Adding aggregation to our language does not affect its expressive power.
In this paper we assume each rule to be \textit{safe}. %i.e., every variable occurring in a rule-head, negative literal or built-in input variable, appears in at least one positive literal of the rule body. 
%As a consequence, we assume all facts to be ground because all not ground fact are not safe. 
A \textit{Datalog$^\neg$ program} $\Pi$ is then a set of safe rules.
%We will sometime employ the function $sch$ to return from a program its schema, i.e., $\mathcal{D} = sch(\Pi).$
As usual we will denote with \textit{edb}$(\mathcal{D})$ and \textit{idb}$(\mathcal{D})$ respectively the \textit{extensional} and the \textit{intensional} part of the database schema. %is the subset of the database schema \textbf{R} containing all relations that appear in at least one rule-head in $\Pi$, while with  $\textit{edb}(\textbf{R}) = \textbf{R} \setminus \textit{idb}(\textbf{R})$ we refer to as the \textit{extensional database}. 
If the program is composed by only positive rules, we refer to it as Datalog, while if negation  appears only in front of \textit{edb} relations -- i.e., $C_j \subseteq edb(\textbf{R})$ -- we will denote it as \textit{semi-positive}, and write Datalog$^{\neg sp}$. If negation is instead allowed also in front of intensional predicates, 
we will employ the \emph{stratified semantics}, and write Datalog$^{\neg s}$.
Finally, if a program is non-recursive, we will use the prefix \emph{Nr}, e.g., NrDatalog$^{\neg sp}$. 
%
%Should we add the fact that we specify with both I and Pi_I a program instance?

\vspace{-1mm}
\begin{ex}
\label{ex:sugared_shortest}
As an introductory example, we use the following program computing all the shortest paths existing between every pair of nodes in a graph. We employ an \textit{edb} relation $L$ containing tuples in the form $(u,v,d)$ to specify the existence of a directed link with length $d$ between a source node $u$ and a destination node $v$. In addition, we employ two intensional relations $P$ and $S$ respectively defining the transitive closure of the relation $L$ -- i.e., all the possible paths -- and the shortest(s) among the paths existing between each pair of source-destination nodes. To identify the shortest(s) path we make use of the $M$ aggregate relation which stores the minimum distance for each source-destination pair. %These four relations \texttt{link}, \texttt{path}, \texttt{shortest} and \texttt{shortestDistance} will remain the same during the entire paper.
%

\vspace{-1mm}
\noindent\hrulefill
\vspace{-1mm}
\small
\begin{equation*}
\begin{split}
&P(u, v, d) \leftarrow L(u, v, d).\\
&P(u, w, d) \leftarrow L(u, v, d1), P(u, w, d2), d = d1 + d2.\\
&M(u, v, min<d>) \leftarrow P(u, v, d).\\
&S(u, v, d) \leftarrow P(u, v, d), M(u, v, d).
\end{split}
\end{equation*}
\noindent\hrulefill
%\vspace{2mm}
\end{ex}
\vspace{-1mm}
\normalsize

==> distributed.tex <==
\stitle{Distributed processing}:
Instantiating a transducer network on top of a physically distributed system is a more difficult exercise than in  the multi-core case.
In fact, although all the transducer nodes can be directly mapped to physical nodes, it is not clear where to map the environment.
This problem can be solved using two different -- not necessarily disjoint -- perspectives: a \emph{logical}, and a \emph{physical} one.
Logically, the environment can be seen as a communication middleware providing both networking and synchronization services.
Physically, the environment can be mapped to a set of networking devices -- \eg switches -- providing the network connectivity where a special software routine is used to synchronize the nodes.
In physically distributed systems, communication is performed using \emph{message passing} and therefore the environment is used to abstract all the low-level details intrinsic in this model.


==> expressiveness.tex <==
%!TEX root = TPLP.tex

In this Appendix we analyze the expressiveness of synchronous transducer networks in computing queries.
In particular we want to address the following question: given a query expressed in a language $\mathcal{L}$, which kind of language $\mathcal{L}^\prime$ can be used internally by a transducer network to implement it in a distributed way? 
%In particular, we are looking for a language $\mathcal{L}^\prime$ which is expressive enough to be employed to compute distributively different languages $\mathcal{L}$, and therefore can be used as a benchmark to measure the complexity in terms of number of rounds that the network need for computing a query.
From \cite{AmelootNB13} we already know that a query is expressible in {\sc datalog} iff it can be distributively computed by an inflationary {\sc nrdatalog}-network:
\begin{proposition}
\label{pr:positive_recursive}
A query is expressible in {\sc datalog} if and only if it can be distributively computed by a broadcasting, inflationary and oblivious {\sc nrdatalog}-network. In addition, the number of rounds is proportional to the number of recursive iterations.
\end{proposition}
Actually, here we are  interested in queries with negation. 
In the next sections we will then fix the lower-bound on $\mathcal{L}^\prime$ to be {\sc fo}, and its upper-bound to be {\sc datalog}$^{\neg}$.
%In addition, we fix {\sc datalog}$^{\neg s}$ as upper-bound for $\mathcal{L}$. 
%In such a way we will be able to express up to \textbf{PSPACE} queries \footnote{Remark that we might have used {\sc datalog}$^{\neg pts}$ as upper-bound, but since past-guarded stratification does not add expressive power to the language, we simply choose {\sc datalog}$^{\neg ts}$.}.
Before continuing the discussion, we have to introduce a remark: we will omit all the cases which fall under Lemma \ref{lm:computable}. %and $(ii)$ in respect to Section \ref{sec:temporal_expressiveness_complexity} we will only consider the expressive power of the distributed system complete evolution. %, i.e., $\mathcal{L} = \mathcal{L}^\prime$.
%The rationale behind $(ii)$ is quite intuitive and is related to the fact that with one transition a query can be evaluated just over the local instance, therefore making the effort of employing a distributed system not general because dependent on the network configuration.
As a notation, in the following we will use $r$ to denote the number of iterations in a recursive program, and $s$ to specify the number of strata in a syntactically stratifiable program. %and finally $t$ to denote the number of temporal steps on a temporal stratifiable program.  

\subsection{Semi-positive Queries}
\label{sec:query_semipositive}

We say that a {\sc datalog}$^\neg$-query is \emph{semi-positive} if every negative literal appearing in the query is over an \emph{edb} relation. 
Henceforth we will then use {\sc datalog}$^{\neg sp}$ to denote  semi-positive {\sc datalog}$^\neg$. 

\begin{proposition}
\label{te:semipositive_recursive}
A query is expressible in {\sc datalog}$^{\neg sp}$ if can be distributively computed by a broadcasting, inflationary and oblivious {\sc fo}-network in O(r) rounds.
\end{proposition}
\begin{proof}
%First we prove the only-if direction.
Denote with $\mathcal{Q}$ the recursive query, and with $\mathcal{D}_{out}$ its output schema.
As in the proof of Lemma \ref{lm:computable}, we can create a transducer $\mathcal{T}$ where all nodes emit their input facts: %which, once received, they are used to  added to the local memory. 
{\sc fo} suffice for this and one round is necessary. After that, we can safely compute $\mathcal{Q}$  because each node has locally the entire initial instance and no wrong fact can be inferred;
$\mathcal{Q}$ however is recursive. The idea here is to employ transducer iterations to implement iterations through recursive predicates.
%Intuitively, the number of rounds is proportional to the number of iterations necessary to exhaust the recursion.
More precisely, let us denote by $\mathcal{T}$ the transducer of case $(ii)$ of Lemma \ref{lm:computable} and with $\mathcal{Q}^\prime$ the version of the query where all the $edb$ relations are now primed and each rule contains the atom \texttt{ready}. 
Being $\mathcal{Q}^\prime$ a {\sc datalog}$^{\neg sp}$ query, we have to develop a mechanism to deal with recursion keeping the transducer in {\sc fo}.
This mechanism comes for free: being the transducer inflationary, once true, \texttt{ready} remains true, therefore if now $Q_{out} = \mathcal{Q}^\prime$ we are able to iterate the query by iterating global transitions, therefore accomplishing recursion.
%Note that $\mathcal{P}$ is indeed a NrDatalog$^{\neg sp}$ program because recursive predicates are in $\mathcal{D}_{out}$ (and therefore in $\Upsilon_{out}$) and hence recursion is expressed by iterating global transitions.
Intuitively, the number of rounds is proportional to the number of iteration necessary to exhaust the recursion.
%The transducer is inflationary.
\end{proof}

\eat{
\begin{example}
Let $\mathcal{Q}$ be the following {\sc datalog}$^{\neg sp}$ query:
\begin{equation*}
\begin{split}
&Q(v, z) \leftarrow R(u, v), Q(u, z), \neg P(u).
\end{split}
\end{equation*}
where $\mathcal{D}_{in}$ and $\mathcal{D}_{out}$ can be inferred in a straightforward way.
A {\sc fo}-transducer computing the same query is:

\noindent\hrulefill
\vspace{-1mm}
\begin{equation*}
\begin{split}
\text{Schema: }&\Upsilon_{db} = \{R^{(2)}, P^{(1)}\},  \Upsilon_{mem} = \{\texttt{ready}^{(0)}\},  \Upsilon_{com} = \{R^{(2)^\prime}, (P^{(1)^\prime}\}, \Upsilon_{out} = \{Q^{(2)}\}\\
\text{Program: }&R^{\prime}_{snd}(u, v) \leftarrow R(u, v).\\
&P^{\prime}_{snd}(u) \leftarrow P(u).\\
&\texttt{ready}_{ins}() \leftarrow \neg \texttt{ready}().\\
%&\texttt{ready}_{ins}() \leftarrow \texttt{init}().\\
&Q_{out}(v, z) \leftarrow R^\prime(u, v), Q(u, z), \neg P^\prime(u), \texttt{ready}().
\end{split}
\end{equation*}
\noindent\hrulefill
\vspace{2mm}
\end{example}
}
%
%\begin{co}
%A query expressed in {\sc datalog}$^{\neg sp}$ can be distributively computed by an inflationary time-space oblivious Nr{\sc datalog}$^{\neg s}$-network in O(r) super-steps
%\end{co}
%

\subsection{Stratified Queries}
\label{sec:query_stratified}

\begin{proposition}
\label{te:stratified}
A query expressed in {\sc nrdatalog}$^{\neg}$ can be distributively computed by a broadcasting, inflationary, and oblivious {\sc fo}-network in O(s) rounds.
\end{proposition}
\begin{proof}
A sequence of {\sc fo} sub-queries $\mathcal{Q}^1, \ldots, \mathcal{Q}^n$ can be obtained from a {\sc nrdatalog}$^{\neg}$ query $\mathcal{Q}$ in a similar way as in the proof of Proposition~\ref{pr:embarassing_non_monotonic}. % \ie each sub-query $\mathcal{Q}^i$ contains the rules defining the $i$-th stratum of $\mathcal{Q}$. %\cite{DBLP:books/aw/AbiteboulHV95}.
%$\mathcal{D}_{out}^i$ is composed by the head relations in $\mathcal{Q}^i_{out}$ which will appear negated in successive sub-queries or that are in $\mathcal{D}_{out}$.
%
%Starting from the transducer $\mathcal{T}$ of Proposition \ref{lm:computable} we can then join all the sub-queries $\mathcal{Q}^1, \ldots, \mathcal{Q}^n$ in a unique output query $Q_{out}$ by appending to each sub-query $\mathcal{Q}^i$ an atom \texttt{stage}$^i$ in order to process in sequence one sub-query per round.
%
%More precisely, let construct a transducer $\mathcal{T}$ identical to the one in case $(ii)$ of Proposition \ref{pr:computable} where however $Q_{out}$ is not defined yet.
%%Let now proceed to insert the sub-queries into the transducer program.
%First, given the sequence $\mathcal{Q}^1, \ldots, \mathcal{Q}^n$ we prime all the $edb$ predicates and append to each rule of sub-query $\mathcal{Q}^i$ the nullary atom \texttt{stage}$^i$.
%Then we add to $\Upsilon_{mem}$ one nullary relation \texttt{stage}$^i$, with $i \in 1, \ldots, n$. %and one relation $R$ for each $R \in idb(\mathcal{Q}) \setminus \mathcal{D}_{out}$. As a consequence we have that $Q_{ins}$ now contains all the rules in $Q_1, \ldots Q_n$ except for the rules defining the output which we add to $Q_{out}$.
%Let add to $Q_{ins}$ a rule in the form of (\ref{eq:stratifed_2}) for each $i, j$, with $1 < i < j \leq n$, and we substitute rule (\ref{eq:computable_4}) with:
%\begin{align}
%\label{eq:stratifed_1}
%&\texttt{stage}^1_{ins}() \leftarrow \neg \texttt{stage}^1(), \neg \texttt{stage}^2, \ldots, \neg \texttt{stage}^n.
%\end{align}
%to define the initial stage.
%%plus a persisting rule in the form of eq. (\ref{eq:semipositive_recursive_7}) for each $R \in idb(\mathcal{Q}) \setminus \mathcal{D}_{out}$.
%%Persisting rules are necessary because an $idb$ relation can be defined at stage $i$ and belonging to the body of a rule of stage $k$, with $k \leq i + 2$.
%%For this reason we made the conservatory choice of persisting all the $idb$ relations not in the output (remark that the output relations are by definition inflationary). 
%We can now add to $Q_{ins}$ all the sub-queries $Q_{out}^i$ when $\mathcal{D}_{out}^i \cap \mathcal{D}_{out} = \emptyset$, and all the rules defining a predicate not in $\mathcal{D}_{out}$, when $\mathcal{D}_{out}^i \cap \mathcal{D}_{out} \neq \emptyset$.
%$Q_{out}$ is composed by all the remaining queries.
The network is clearly inflationary, oblivious and the execution time is proportional to the number of strata.
%The network can be easily made inflationary by persisting each \texttt{ready}$^i$ and each \texttt{stage}$^j$.
%The inflationary version of $\mathcal{P}$ is more correct in respect to the one used in the proof because it avoiding infinite cycles. 
%We described the non-inflationary version because it will result useful for proving the next theorems.
\end{proof}
%
\begin{corollary}
A query expressed in {\sc datalog}$^{\neg}$ can be distributively computed by a broadcasting, inflationary, and oblivious {\sc datalog}$^{\neg sp}$-network in O(s) rounds.
\end{corollary}
%
Let us denote with $r_i$ the number of recursive iterations inside stratum $i$ before the  stratum is exhausted.
If we assume $R = \sum_{i \in 1, \ldots, s}r_i$, we have the followings:
\begin{proposition}
\label{te:stratified_recursive_semipositive}
A query expressed in {\sc datalog}$^{\neg}$ can be distributively computed by a broadcasting and oblivious {\sc nrdatalog}$^{\neg sp}$-network in O(s + R) rounds.
\end{proposition}
\begin{proof}
The proof of this Proposition follows from the proof of Propositions~\ref{te:stratified} and \ref{pr:embarassing_non_monotonic} with some small modifications.
The idea here is again to divide the program into strata.
A stratum cannot start until the previous one is terminated. Thus, since a stratum can now be recursive but computation within each stratum is monotone, it is sufficient to check whether some predicate is currently true, whereas it was false in the previous state.

To be more precise, assume $\mathcal{Q}^1, \ldots, \mathcal{Q}^n$ to be a stratification of $\mathcal{Q}$. 
Consider the transducer $\mathcal{T}$ derived from $\mathcal{Q}^1, \ldots, \mathcal{Q}^n$ as in Proposition \ref{te:stratified}.
From $\mathcal{T}$ we can now derive a new transducer $\mathcal{T}^\prime$ by adding to $\Upsilon_{mem}$ a predicate $R^{old}$ for each recursive predicate $R \in idb(\mathcal{Q})$ plus a nullary relation $\texttt{stage}^{old\text{ }i}$ %, $\texttt{stage}^i$ 
for each sub-query $\mathcal{Q}^i$ having at least a recursive predicate.
We can now modify $Q_{ins}$ by adding a pair of rules:
\begin{align}
\label{eq:stratified_recursive_1}
&R^{old}_{ins}(\bar{u}) \leftarrow R(\bar{u}), \texttt{stage}^i().\\
\label{eq:stratified_recursive_2}
&\texttt{stage}^i_{ins}() \leftarrow R(\bar{u}), \neg R^{old}(\bar{u}), \texttt{stage}^i().
\end{align}
for each recursive predicated $R \in idb(\mathcal{Q}^i_{out})$ in order to detect if a recursive rule exists that has created new facts between two consecutive evaluations of the $i$-th stage.
In addition, in order to transit between stages we make use of the rules:
\begin{align}
\label{eq:stratified_recursive_3}
&\texttt{stage}^{old\text{ }i}_{ins}() \leftarrow \texttt{stage}^i().\\
\label{eq:stratified_recursive_4}
&\texttt{stage}^i_{del}() \leftarrow \texttt{stage}^i().\\
\label{eq:stratified_recursive_5}
&\texttt{stage}^j_{ins}() \leftarrow \texttt{stage}^{old\text{ }i}(), \neg \texttt{stage}^i().
\end{align}
so that a new stage will start only when the current stage has finished in the present round while was active in the previous one.
This mechanism in needed because two super-steps are necessary to fill in the $R^{old}$ relation and detect if new facts have been derived.
%In addition we substitute eq. (\ref{eq:computable_5}) with
%\begin{align}
%\label{eq:stratified_recursive_semipositive_6}
%&\texttt{stage}^1_{ins}() \leftarrow \texttt{init}().
%\end{align}
%in order to start the first stage.
Intuitively, since we employed Theorem \ref{te:stratified} for stratification, and recursion may exists in each stratum, the number of rounds is proportional to the number of strata plus the total number of recursive iterations.
\eat{
\begin{ex}[NrDatalog$^{\neg sp}$-network Computing a Datalog$^{\neg s}$-query]
Let $\mathcal{Q}_{out}$ be the following Data\-log$^{\neg s}$ query: 
\begin{equation*}
\begin{split}
&T(u, v) \leftarrow R(u, v), \neg P(u).\\
&T(v, z) \leftarrow R(u, v), T(u, z), \neg P(u).\\
&Q(v, z) \leftarrow R(u, v), \neg T(u, z).
\end{split}
\end{equation*}
where $\mathcal{D}_{in} = \{R, P\}$ and $\mathcal{D}_{out} = Q$.
A NrDatalog$^{\neg s}$ transducer computing the same query is:

\noindent\hrulefill
\vspace{-1mm}
\begin{equation*}
\begin{split}
\text{Schema: }&\mathcal{T}_{db} = \{(R, 2), (P, 1)\},  \mathcal{T}_{mem} = \{(T^{old}, 2), (\texttt{stage}^1, 0), (\texttt{stage}^{old \text{ }1}, 0),\\&(\texttt{stage}^2, 0), (\texttt{stage}^{old \text{ }2}, 0), (T, 2)\}, \mathcal{T}_{sync} = \{(R^{\prime}, 2), (P^{\prime}, 1)\}, \\&\mathcal{T}_{out} = \{(Q, 2)\}\\
\text{Program:}&\\
\end{split}
\end{equation*}
\vspace{-3mm}
\begin{equation*}
\begin{split}
%&R^{sync}_{emt}(\texttt{u}, \texttt{v}) \leftarrow R(\texttt{u}, \texttt{v}).\\
%&P^{sync}_{emt}(\texttt{u}) \leftarrow P(\texttt{u}).\\
%&R^{\prime}_{ins}(\texttt{u}, \texttt{v}) \leftarrow R^{sync}(\texttt{u}, \texttt{v}).\\
%&P^{\prime}_{ins}(\texttt{u}) \leftarrow P^{sync}(\texttt{u}).\\
&R^{\prime}_{emt}(u, v) \leftarrow R(u, v).\\
&P^{\prime}_{emt}(u) \leftarrow P(u).\\
%&\texttt{init}_{ins}() \leftarrow \neg \texttt{init}().\\
&\texttt{stage}^1_{ins}() \leftarrow \neg \texttt{stage}^1(), \neg \texttt{stage}^2().\\
&\texttt{stage}^{old\text{ }1}_{ins}() \leftarrow \texttt{stage}^1().\\
&\texttt{stage}^{1}_{del}() \leftarrow \texttt{stage}^1().\\
&\texttt{stage}^2_{ins}() \leftarrow \texttt{stage}^{old\text{ }1}(), \neg \texttt{stage}^{1}().\\
%&\texttt{stage}^{1}_{ins}() \leftarrow \texttt{stage}^2().\\
%&\texttt{stage}^{old \text{ }1}_{del}() \leftarrow \texttt{stage}^2().\\
&T^{old}_{ins}(u, v) \leftarrow T(u, v), \texttt{stage}^1().\\
&\texttt{stage}^1_{ins}() \leftarrow T(u, v), \neg T^{old}(u, v), \texttt{stage}^1().\\
&T_{ins}(u, v) \leftarrow R^\prime(u, v), \neg P^\prime(u), \texttt{stage}^1().\\
&T_{ins}(v, z) \leftarrow R^\prime(u, v), T(u, z), \neg P^\prime(u), \texttt{stage}^1().\\
&Q_{out}(v, z) \leftarrow R^\prime(u, v), \neg T(u, z), \texttt{stage}^2().
\end{split}
\end{equation*}
\noindent\hrulefill
\vspace{2mm}
\end{ex}
}
\end{proof}
%by substituting the appropriate rule in the form of eq. \ref{eq:steps} with the following rules:
%\begin{align}
%\label{eq:steps}
%\texttt{step}^j_{ins}() \leftarrow \texttt{step}^{\prime i}().
%\end{align}
%\end{itemize}
%
%
\noindent Because a stratified program may have many different stratifications, from the above theorems clearly follows that, if {\sc fo}-{\sc datalog}$^{\neg sp}$ is chosen as transducer network language, among all the possible stratifications the ones with the minimum number of strata should be preferred: 
%
\begin{corollary}
A query expressed in {\sc datalog}$^{\neg}$ can be distributively computed by a broadcasting, and oblivious {\sc nrdatalog}$^{\neg}$-network in O(s + R) rounds.
\end{corollary}

\subsection{Beyond Stratified Queries}
\label{sec:expres_discussion}

We have seen that, by tuning the transducer type, we are also able to tune the expressive power of a transducer.
In particular, we have shown that an inflationary oblivious transducer is able to compute up to {\sc datalog}$^{\neg sp}$ -- also known to be equivalent to \emph{existential least fixpoint logic} $E(LFP)$ \cite{DBLP:books/daglib/0082516} -- if $\mathcal{L}^\prime =$ {\sc fo}.
If instead we set $\mathcal{L}^\prime =$ {\sc datalog}$^{\neg sp}$ we can express up to {\sc datalog}$^{\neg}$ queries.
But which is the general expressive power of inflationary transducers?
As stated by the following proposition, we are able to express up to \textsc{fixpoint}.
%
\begin{proposition}
A query is expressible in \textsc{fixpoint} if and only if can be distributively computed by an inflationary, disseminating, and oblivious broadcasting transducer network.
\end{proposition}
\begin{proof}
For the if direction we have to show that we are able to express any {\sc datalog}$^{\neg}$-query $\mathcal{Q}$ under the inflationary semantics \cite{AbiteboulHV95}, with an inflationary disseminating transducer network:
it is in fact known that {\sc datalog}$^{\neg}$ with inflationary semantics is equivalent to \textsc{fixpoint} \cite{AbiteboulHV95}.
We can use the same approach illustrated in the proof of Proposition \ref{te:stratified_recursive_semipositive} which installs every query composing $\mathcal{Q}$ in $Q_{out}$ with appended the goal \texttt{ready}$()$.

For the only-if direction, let $\mathcal{N}$ be an inflationary disseminating and oblivious transducer distributively computing a query $\mathcal{Q}_{out}$. 
We have to show that $\mathcal{Q}_{out}$ can be computed by a {\sc datalog}$^{\neg}$-program with inflationary semantics. 
We can union all the rules of the transducer program $\mathcal{P}$ in a {\sc datalog}$^{\neg}$ program $\Pi$.
Let us consider as canonical model of $\Pi$ the inflationary semantics. %, i.e., $\Pi$ is a {\sc datalog}$^{\neg+}$-program.
$\Pi$ and $\mathcal{N}$ have the same opportunity of eventually deriving a fact. %and, in the opposite way, $\mathcal{N}$ generate the same facts of $\Pi$.
To see why this is the case, consider a trivial configuration for $\mathcal{N}$ (remember that $\mathcal{N}$ is independent because distributively computing a query). 
In such situation every emitted fact is employed by the same node in the successive transition, and every derived fact will never be deleted because the transducer network is inflationary.
We can hence conclude that $\Pi$ and $\mathcal{N}$ compute the same query.
\end{proof}
%
\noindent Note the fact that the transducer network must be disseminating.
Indeed, being a transducer disseminating, tuple sending is inflationary: given two database instances \textbf{I}, \textbf{J}, with $\textbf{I} \subseteq \textbf{J}$, we have that $Q_{snd}(\textbf{I}) \subseteq Q_{snd}(\textbf{J})$.
If the transducer is not disseminating -- \eg we emit facts after been previously used by other rules -- the same property doesn't hold.

If instead we consider non-inflationary oblivious networks, we are able to express {\sc datalog}$^{\neg}$ even if $\mathcal{L}^\prime =$ {\sc fo}.
%This is due to the fact that $Q_{del}$ queries are necessary to detect if a recursive stage is terminated and hence the next one can be activated.
In the non-inflationary case, we have that specifications (not necessarily disseminating) can express up to \textsc{while}.
%Then, in addition of inflationary and non-inflationary networks, we have also employed semi-inflationary networks.
%In particular, we have shown that a semi-inflationary oblivious transducer is able to compute {\sc datalog}$^{\neg s}$, but what is its limit?
%
\begin{proposition}
\label{pr:semi_inflationary_while}
A query is expressible in \textsc{while} if and only if can be distributively computed by an oblivious and broadcasting transducer network.
\end{proposition}
\begin{proof}
Starting from the if direction, we can compute a {\sc datalog}$^{\neg}$-query with non-inflationary (or partial) semantics~\cite{DBLP:books/daglib/0082516}with a non-inflationary network by using just memory relations and output the result just when we have detected that the computation is finished.
The specification of such transducer implements exactly the partial fixpoint operator computation.
More precisely, let $\mathcal{T}$ the transducer network generated from $\mathcal{Q}$ following the procedure depicted in Lemma \ref{lm:computable}, but where, this time, all the rules are installed in $Q_{ins}$ with every predicate in $\mathcal{D}_{out}$ primed, $Q_{del}$ deletes the content of every $memory$ relation, while $Q_{out}$ is composed of  one rule in the following form:
\begin{equation}
R_{out}(\bar{u}) \leftarrow R^{prev}(\bar{u}), \neg \texttt{change}().
\end{equation}
for each predicate $R \in \mathcal{D}_{out}$, and where the nullary predicate \texttt{change} is true every time two consecutive iterations have different states.
It remains to specify how we can detect that the computation is terminated and therefore the result can be output (\ie the rules defining the predicate \texttt{change}).

To do this, we add a new set of rules to $Q_{ins}$:
\begin{align}
\label{eq:partial_1}
&\texttt{ready}_{ins}() \leftarrow \texttt{ready}().\\
%&\texttt{done}_{ins}() \leftarrow \texttt{ready}().\\
%&\texttt{done}_{ins}() \leftarrow \texttt{done}().\\
\label{eq:partial_2}
&R^{prev}_{ins}(\bar{u}) \leftarrow R^{\prime}(\bar{u}).\\
\label{eq:partial_3}
&\texttt{change}() \leftarrow R^{prev}(\bar{u}), \neg R^{\prime}(\bar{u}), \texttt{ready}().\\
\label{eq:partial_4}
&\texttt{change}() \leftarrow \neg R^{prev}(\bar{u}), R^{\prime}(\bar{u}), \texttt{ready}().
\end{align}
where $(\ref{eq:partial_1})$ is used so that the initial instance is employed only for the first iteration; $(\ref{eq:partial_2})$ defines the previous version of relation $R^{\prime}$, and is employed in rules $(\ref{eq:partial_3})$ - $(\ref{eq:partial_4})$ to derive when two consecutive states are identical.
%For the only-if direction, let $\mathcal{N}^b$ be a semi-inflationary and oblivious transducer distributively computing a query $\mathcal{Q}_{out}$. 
%We have to show that $\mathcal{Q}_{out}$ can be computed by a {\sc datalog}$^{\neg -}$-program. 
%We can join all the rules of the transducer program $\mathcal{P}$ in a {\sc datalog}$^{\neg}$ program $\Pi$.
%In order to implement the semi-inflationary semantics, we then must add a persistent rule in the form of eq. (\ref{eq:temp_persist}) for every $memory$ and $output$ relation.
%Let consider as canonical model of $\Pi$ the sem-inflationary semantics, i.e., $\Pi$ is a {\sc datalog}$^{\neg+}$-program.
%$\Pi$ and $\mathcal{N}$ have the same opportunity of eventually deriving a facts. %and, in the opposite way, $\mathcal{N}$ generate the same facts of $\Pi$.
%To see why this is the case, consider a trivial configuration for $\mathcal{N}^b$ (remember that $\mathcal{N}^b$ is independent because distributively computing a query). 
%In such situation every emitted fact is employed by the same node in the successive transition. %and every derived fact will never be deleted because the transducer network is inflationary.
%We can hence conclude that $\Pi$ and $\mathcal{N}^b$ compute the same query $Q_{out}$.

We now consider the only-if direction. We can follow the same procedure as in the proof of Lemma 6.1 in \cite{AmelootNB13}.
Let $\mathcal{N}$ be an oblivious, non-inflationary and broadcasting {fo}-transducer network over a schema $\Upsilon$, distributively computing a query $\mathcal{Q}$. We show that $\mathcal{Q}$ can be computed by a {\sc while}-program $\Pi$. Because of network-independence, it is sufficient to look at the behavior of $\mathcal{N}$ on a single-node network. 
Intuitively the while loop composing $\Pi$ simulates the computational rounds of $\mathcal{N}$.
$\Pi$ schema contains a relation $R_{del}$ for every $R \in \Upsilon_{mem}$, whose semantics is defined by the related $Q_{del}$-query.
$\Pi$ contains every query in $Q_{ins}$ defining $R$ augmented with a new goal $\neg R_{del}(\bar{u})$.
$\Pi$ finally contains all the remaining rules in $\mathcal{P}$. 
Finally we add a specific rule for each $database$ relation, implementing the persistent semantics over database facts.
$\Pi$ has the same opportunity of $\mathcal{N}$ to eventually derive facts.
The {\sc while}-program $\Pi$ terminates exactly when two consecutive iterations has the same state, exactly as the definition of network quiescence in Section~\ref{sec:sync_computability}.
\end{proof}
%\noindent From the above properties follows that semi- and non-inflationary networks have the same expressive power since non-inflationary networks are able to express {\sc datalog}$^{\neg ts}$-queries by Theorem \ref{te:temporal_recursive} and they are clearly not able to brake the \textbf{PSPACE} barrier since neither $(i)$ variable-arity relations are allowed, nor $(ii)$ new constants can be created.  
%We can hence conclude that choosing one or the other layout is just a matter convenience. 
%The reader should not be surprised by this result: indeed non-inflationary queries can be implemented by a semi-inflationary network and vice-versa. %by pushing the evaluation of the actual query from $Q_{out}$ to $Q_{ins}$, and by setting $Q_{del}$ to delete in every transition all the facts.
%
%The next theorem show that the limit of semi-inflationary transducer is \textsc{fixpoint}.
%\begin{te}
%A query is expressible in {\sc datalog}$^{\neg ws}$ if and only if can be distributively computed by a semi-inflationary time-space oblivious Nr{\sc datalog}$^{\neg sp}$-network
%\end{te}
%\begin{proof}
%For the only-if part we show that win-move is expressible using a semi-inflationary time-space oblivious Nr{\sc datalog}$^{\neg sp}$-network.
%check pag 85 statelog
%\end{proof}
%
%Finally, we have also see that a (non-inflationary) time-space oblivious network is able to implement up to \textsc{while}.


%Quite a few combinations of $\mathcal{L}$ and $\mathcal{L}^\prime$ exist.
%Fixed a query expressed in a certain language $\mathcal{L}$, we can tune the \emph{granularity} of the task by appropriately choosing the network implementation language $\mathcal{L}^\prime$, where, intuitively, a less expressive language correspond to fine-grained tasks.
%By selecting fine-grained tasks, the user would also be able to exploit \emph{partial results} as the computation proceeds and therefore having a more interacting experience, as required by today data-analysis tools \cite{Condie:2010:MO:1855711.1855732}, instead of a one shot program. 

%From a fault tolerance perspective, if we assume a checkpointing model -- i.e., the full global state is saved in persistent memory so that, in case of failures, the computation can restart from a checkpoint and not from the beginning -- by tuning the granularity of tasks we can also tune the checkpointing frequency. 
%Thus, for example, if in a recursive query we want to visualize and save partial results, then $\mathcal{L}^\prime$ should be set to be non recursive. %as shown in Example \ref{non_recursive_tc}.
%In addition, more aggressive checkpointing strategies can be implemented.
%For instance, a global state checkpoint can be set with low frequency, while among global checkpoints just the local state of the environment can be saved. In fact, since local transitions are deterministic, given a global state and a sequence of input instance -- which are part of the environment local state -- the sequence of global states can be reconstructed.
%This technique is somehow similar to the lineage model implemented in Spark \cite{Zaharia:2012:RDD:2228298.2228301}.

==> relaxing_simultaneity.tex <==
\stitle{Discussion}: From a practical perspective, not all the assumptions we made are easy to implement as in multi-core settings.
Although some of them are realistic, other are less realistic and therefore can be relaxed.
Among the more realistic ones, there is the reliability assumption of the communication medium, which, even in networked system, can be naturally enforced by using proper protocols.
On the other side, it seems pretty unreasonable in networked systems to have an entity collecting all the emitted tuples (the environment in our model). 
As already mentioned, this is a high-level abstraction useful for reasoning about the distributed computation. %although realistic perspectives for this abstraction exist.
Furthermore, in general the assumption of simultaneity among local transitions can be relaxed: a transducer which has not been fired yet in the current round is randomly chosen and fired. A global transition is then accomplished when all the transducers have been fired exactly once. 
To avoid situations in which no transducer is fired, a \emph{fairness} condition can be imposed on global transitions: each transducer is eventually fired at least once in each round.
This is how most parallel models work in practice: processes execute their computation and wait until all the other have finished. %\ie the synchronization barrier has been reached.

%In addition, instead of relying on an external tape providing the clock for the computation, we can employ the environment to directly supply the computing nodes with the proper time-step. 
%To accomplish that, we have that $\mathcal{T}^e_{mem}$ now contains a new relation \texttt{time} and $\mathcal{P}^e$ is composed by the following clauses:
%\begin{align}
%&\texttt{time}(\texttt{s}) \leftarrow \texttt{time}(\texttt{t}), \texttt{succ}(\texttt{t}, \texttt{s}).\\
%&\texttt{time}(0).
%\end{align}
%where (11) is used to move forward the current round, while (12) inject into the program the starting round.
%A global transition, now denoted by $\textbf{I} {\Rightarrow} \textbf{J}$, is exactly as in Section \ref{sec:global_transitions} but where now, instead of the tape, the \texttt{time} relation provide directly the clock value $t$. 
%From a practical perspective, the assumption of simultaneity can be relaxed in the following way: a round is divided in $n$, with $n = |L|$, concurrent steps which can be fired asynchronously in whichever order. Each of the $1 \leq i \leq n$ steps performs a local transition for a node randomly chosen among the $L - \bigcup_j f(j)$ not yet fired nodes, where $f$ is a function mapping each already computed step with the associated node. In addition, for each step $j$, the environment accomplish a \emph{partial local transition} i.e., a transition related only to a partition of the input, namely the partition computed by the $f(j)$ timed transducer. More formally, if $I_{in}^{e/i} = J^i_{com} \cup J_{out}^i$, then a partial local transition is defined by ($\textbf{I}^e$, $I_{in}^{e/i}$, ${\Longrightarrow} \textbf{J}^{e/i}$, $J^{e/i}_{out})$.
%all the tuples $J_{com}^{f(j)}$ and $J_{out}^{f(j)}$ are accumulated in the next environment state.
%The remaining step is used to compute the output query, which indeed is independent from the other $n$ steps because they both modify only the next states.
%At the end of the $n$ steps, we have that all the transducers have finished their computation, and that $J_{mem}^{e} = \bigcup_{i \in L} J_{mem}^{e/i}$, $J_{out}^{e} = \bigcup_{i \in L} J_{out}^{e/i}$ are properly filled, therefore finishing the round.
%\vspace{20mm}
